CAFe: Unifying Representation and Generation with Contrastive-Autoregressive Finetuning

The rapid advancement of large vision-language models (LVLMs) has driven significant progress in multimodal tasks, enabling models to interpret, reason, and generate outputs across both visual and textual domains. While excelling in generative tasks, existing LVLMs often face limitations in tasks requiring high-fidelity representation learning, such as generating image or text embeddings for retrieval. Recent work has proposed finetuning LVLMs for representational learning, but the fine-tuned model often loses its generative capabilities due to the representational learning training paradigm. To address this trade-off, we introduce CAFe, a contrastive-autoregressive fine-tuning framework that enhances LVLMs for both representation and generative tasks. By integrating a contrastive objective with autoregressive language modeling, our approach unifies these traditionally separate tasks, achieving state-of-the-art results in both multimodal retrieval and multimodal generative benchmarks, including object hallucination (OH) mitigation. CAFe establishes a novel framework that synergizes embedding and generative functionalities in a single model, setting a foundation for future multimodal models that excel in both retrieval precision and coherent output generation.

==> sec/0_abstract.tex <==
\begin{abstract}
The rapid advancement of large vision-language models (LVLMs) has driven significant progress in multimodal tasks, enabling models to interpret, reason, and generate outputs across both visual and textual domains. 
%
While excelling in generative tasks, existing LVLMs often face limitations in tasks requiring high-fidelity representation learning, such as generating image or text embeddings for retrieval. 
%
Recent work has proposed finetuning LVLMs for representational learning, but the finetuned model often loses its generative capabilities due to the representational learning training paradigm.
%
To address this trade-off, we introduce \textbf{\algname}, a \textbf{c}ontrastive-\textbf{a}utoregressive \textbf{f}in\textbf{e}-tuning framework that enhances LVLMs for both representation and generative tasks.
%
By integrating a contrastive objective with autoregressive language modeling, our approach unifies these traditionally separate tasks, achieving state-of-the-art results in both multimodal retrieval and multimodal generative benchmarks, including
%  visual question answering (VQA) and 
object hallucination (OH) mitigation. 
%
% To the best of our knowledge, 
\algname establishes a novel
% the first 
framework that synergizes embedding and generative functionalities in a single model, setting a foundation for future multimodal models that excel in both retrieval precision and coherent output generation.
%
\end{abstract}
